Methods for Combining and Representing Non-Contextual Autonomy Scores for Unmanned Aerial Systems

Measuring an overall autonomy score for a robotic system requires the combination of a set of relevant aspects and features of the system that might be measured in different units, qualitative, and/or discordant. In this paper, we build upon an existing non-contextual autonomy framework that measures and combines the Autonomy Level and the Component Performance of a system as overall autonomy score. We examine several methods of combining features, showing how some methods find different rankings of the same data, and we employ the weighted product method to resolve this issue. Furthermore, we introduce the non-contextual autonomy coordinate and represent the overall autonomy of a system with an autonomy distance. We apply our method to a set of seven Unmanned Aerial Systems (UAS) and obtain their absolute autonomy score as well as their relative score with respect to the best system.

==> extras.tex <==


%To calculate the $N_{CP}$ using existing information, we have designed a set of tables that enable us to compare each architecture layer (including perception, modeling, planning, and execution) on a scale of 1 to 3. In each layer, we assigned three levels including a minimum to achieve autonomy (Level 1), the expected requirements to achieve autonomy (Level 2), and exceeding requirements to achieve autonomy (Level 3). Platforms which receive level 3 evaluations have the capability for more autonomy than those at lower levels. The following tables represent the designed levels in each architecture level. In Table~\ref{tab:component-table}, some terms presented are not self-explanatory and will be defined here. For obstacle detection and avoidance, limited and full depend upon the complexity of algorithms in place. For example, some systems model the environment with obstacles and plans a path around those obstacles. Other systems may only visually detect an obstacle in front of them and plan a partial path in an attempt to avoid the obstacle. Additionally, semi-autonomous execution is execution which still needs an operator, while in full autonomous execution no operator is needed. Results of the component performance evaluation can be seen in Table~\ref{tab:N-CP-table}. Here, levels for each of the four layers are assigned an individual score according to the average of the criteria met in Table~\ref{tab:component-table}. Finally, a value for $N_{CP}$ is found by summing the individual scores. We also show the area captured in the radar chart (shown in Fig.~\ref{fig:radar}) as another metric to represent the total component score.


%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMENT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{table}[ht]
\centering
\scriptsize
\caption{\small{Component requirements for each of the four layers.}}
\label{tab:component-table}
\begin{tabular}{|l|l|l|l|l|}
\hline
\multirow{4}{*}{\textbf{Perception}} &         & \textbf{\begin{tabular}[c]{@{}l@{}} \# Proprioceptive \\ Sensors\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}\# Exteroceptive \\ Sensors\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Type of \\ Camera\end{tabular}}            \\ \cline{2-5} 
                                     & Level 1 & 1 or less                                                                               & 1 or less                                                                              & Thermal/EO                                                                    \\ \cline{2-5} 
                                     & Level 2 & 2-3                                                                                     & 2-3                                                                                    & RGB                                                                           \\ \cline{2-5} 
                                     & Level 3 & 4 or more                                                                               & 4 or more                                                                              & Video                                                                         \\ \hline
\multirow{4}{*}{\textbf{Modeling}}   &         & \multicolumn{2}{l|}{\textbf{Obstacle Detection}}                                                                                                                                 & \textbf{Mapping}                                                              \\ \cline{2-5} 
                                     & Level 1 & \multicolumn{2}{l|}{None}                                                                                                                                                        & None                                                                          \\ \cline{2-5} 
                                     & Level 2 & \multicolumn{2}{l|}{Limited Obstacle Detection}                                                                                                                                  & 2D                                                                            \\ \cline{2-5} 
                                     & Level 3 & \multicolumn{2}{l|}{Full Obstacle Detection}                                                                                                                                     & 3D                                                                            \\ \hline
\multirow{4}{*}{\textbf{Planning}}   &         & \multicolumn{2}{l|}{\textbf{Obstacle Avoidance}}                                                                                                                                 & \textbf{\begin{tabular}[c]{@{}l@{}} Navigation System\end{tabular}} \\ \cline{2-5} 
                                     & Level 1 & \multicolumn{2}{l|}{None}                                                                                                                                                        & None                                                                          \\ \cline{2-5} 
                                     & Level 2 & \multicolumn{2}{l|}{Limited Obstacle Avoidance}                                                                                                                                  & Visual or GPS                                                                 \\ \cline{2-5} 
                                     & Level 3 & \multicolumn{2}{l|}{Full Obstacle Avoidance}                                                                                                                                     & Both GPS and Visual                                                           \\ \hline
\multirow{4}{*}{\textbf{Execution}}  &         & \multicolumn{3}{l|}{\textbf{Execution Ability}}                                                                                                                                                                                                                  \\ \cline{2-5} 
                                     & Level 1 & \multicolumn{3}{l|}{No Autonomous Execution}                                                                                                                                                                                                                     \\ \cline{2-5} 
                                     & Level 2 & \multicolumn{3}{l|}{Semi-Autonomous Execution}                                                                                                                                                                                                                   \\ \cline{2-5} 
                                     & Level 3 & \multicolumn{3}{l|}{Full Autonomous Execution}                                                                                                                                                                                                                   \\ \hline
\end{tabular}
\end{table}


\begin{table}[ht]
\centering
\scriptsize
\caption{\small{Evaluations of components for each system.}}
\label{tab:N-CP-table}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Platform} & \textbf{\begin{tabular}[c]{@{}c@{}}Perception\\ Level\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Modeling\\ Level\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Planning\\ Level\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Execution\\ Level\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Sum\end{tabular}} &
\textbf{\begin{tabular}[c]{@{}c@{}}Figure\\ Area\end{tabular}}\\ \hline
UAS A & 2 & 3 & 2.5 & 3 & 10.5 & 13.5 \\ \hline
UAS B & 3 & 3 & 2 & 2 & 10 & 12.5 \\ \hline
UAS C & 2 & 1 & 1 & 1 & 5 & 3 \\ \hline
UAS D & 2 & 2 & 1.5 & 2 & 7.5 & 7 \\ \hline
UAS E & 3 & 3 & 3 & 3 & 12 & 18 \\ \hline
UAS F & 2 & 1.5 & 2 & 2 & 7.5 & 7 \\ \hline
UAS G & 2 & 1.5 & 1.5 & 2 & 7 & 6.13 \\ \hline
\end{tabular}
\end{table}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%% COMMENT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\begin{comment}

\begin{figure}[h]
\centering
\includegraphics[width=0.48\textwidth]{Figures/autonomy_diff_uniform_weights.png}
\includegraphics[width=0.48\textwidth]{Figures/autonomy_diff_new_weights.png}
\caption{\small{Autonomous differential (AD) of each system with respect to UAS E, plotted one dimensionally. These evaluations show relative autonomy of systems compared to each other. Two weighting methods are shown, uniform weights (left) and normalized weights (right).}}
\label{fig:autonomy_diff_plot}
\end{figure}

\end{comment}
%\bigskip

%that the has a poor component performance test scores. Note that according to NCAP, a UAS that fails 100\% of the time at its mission, but is operated fully autonomously would still have a combined NCAP score of $N=3.0$. It also should be noted that the combined NCAP score does not provide an evaluation of a UAS’s autonomous performance, it, however, encapsulates a UAS’s potential to operate autonomously. 
%Using current information and evaluations explained up to this point, we calculate a preliminary combined NCAP score. To calculate $N_{CP}$, we use the sum of the component performance scores in each layer and then normalize them. We then calculate the NCAP score N,  simply by adding  $N_{CP}$ to the UAS autonomy level $N_{AL}$. The the NCAP score N for each platform are listed in the following table:
\begin{comment}

\begin{table}
\begin{minipage}{.70\linewidth}
\centering
\scriptsize
\label{tab:ncp-score-table-equal}
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{\textbf{Platform}} &
$S_{max}$ & $S_{map}$ & $S_{zsc}$ & $S_{sum}$ & $P$ & $N_{AL}$ \\ \midrule
UAS A & 0.184 (6) & 0.326 (5) & -0.984 (7) & 0.049 (7) & 2.479 (6) & 3 \\ 
UAS B & 0.170 (7) & 0.296 (7) &	0.222 (2) & 0.051 (6) & 2.291 (7) & 1 \\ 
UAS C & 0.203 (6) & 0.296 (6) & -0.093 (5) & 0.061 (5) & 2.595 (5) & 0 \\
UAS D & 0.349 (2) & 0.495 (4) & 0.048 (4) & 0.094 (4) & 3.484 (4) & 3 \\ 
UAS E & 0.528 (1) & 0.724 (1) & 0.927 (1) & 0.142 (1) & 4.634 (1) & 3	\\
UAS F & 0.394 (3) & 0.566 (2) & 0.049 (3) & 0.102 (3) & 3.806 (2) & 0	\\
UAS G & 0.384 (5) & 0.522 (3) & -0.274 (6) & 0.103 (2) & 3.558 (3) & 0 \\
\bottomrule
\end{tabular}
\caption{\small{Component performance ($N_{CP}$) for each platform using different combination methods and uniform weights.}}
\end{minipage}%
\hspace{\fill}
%\end{table}
%\begin{figure}[htbp]
\begin{minipage}{.28\linewidth}
\centering
\includegraphics[width=\textwidth]{Figures/ncp_rankings_equal.png}
\captionof{figure}{\small{UAS platform rankings and $N_{CP}$ scores obtained by different combining methods. }}%Each circle represents an $N_{CP}$ score for a specific UAS. Bigger circles correlate to higher ranks. The vertical lines show the range of scores for each method. The weighted product results have been represented separately because of the shift in the values.}}
\label{fig:rankings-chart-equal}
\end{minipage}
\end{table}
\end{comment}
%\end{figure}




\begin{comment}

%\end{minipage}
\vspace{-1em}
\hspace{\fill}
\vspace{-1em}
\begin{minipage}{.45\linewidth}
\centering
\scriptsize
\caption{\small{UAS platform rankings based on $N_{CP}$ scores obtained by different combining methods}}
\label{tab:ncp-rankings-table}
\begin{tabular}{lccccc}
\toprule
\multicolumn{1}{c}{\textbf{Platform}} &
$S_{max}$ & $S_{map}$ & $S_{zsc}$ & $S_{sum}$ & $P$
\\ \midrule
UAS A & 5 &  5 & 6 & 6 & 5 \\
UAS B & 6 & 6 & 3 & 5 & 6 \\ 
UAS D & 4 & 4 & 5 & 4 & 4 \\ 
UAS E & 1 & 1 & 1 & 1 & 1	\\ 
UAS F & 2 & 2 & 4 & 3 & 2	\\ 
UAS G & 3 & 3 & 2 & 2 & 3\\ 
\bottomrule

\end{tabular}
\end{minipage}
%\end{table}
\end{comment}
%\vspace{1em}


\begin{comment}


\begin{table}
\centering
\scriptsize
\caption{\small{Component performance ($N_{CP}$) for each platform using different combination methods and uniform weights.}}
\label{tab:ncp-score-table-equal}
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{\textbf{Platform}} &
$S_{max}$ & $S_{map}$ & $S_{zsc}$ & $S_{sum}$ & $P$ & $N_{AL}$ \\ \midrule
UAS A & 0.184 (6) & 0.326 (5) & -0.984 (7) & 0.049 (7) & 2.479 (6) & 3 \\ 
UAS B & 0.170 (7) & 0.296 (7) &	0.222 (2) & 0.051 (6) & 2.291 (7) & 1 \\ 
UAS C & 0.203 (6) & 0.296 (6) & -0.093 (5) & 0.061 (5) & 2.595 (5) & 0 \\
UAS D & 0.349 (2) & 0.495 (4) & 0.048 (4) & 0.094 (4) & 3.484 (4) & 3 \\ 
UAS E & 0.528 (1) & 0.724 (1) & 0.927 (1) & 0.142 (1) & 4.634 (1) & 3	\\
UAS F & 0.394 (3) & 0.566 (2) & 0.049 (3) & 0.102 (3) & 3.806 (2) & 0	\\
UAS G & 0.384 (5) & 0.522 (3) & -0.274 (6) & 0.103 (2) & 3.558 (3) & 0 \\
\bottomrule
\end{tabular}
\end{table}

%\vspace{-1em}
\begin{table}[ht]
%\begin{minipage}{.45\linewidth}
\centering
\scriptsize
\caption{\small{Component performance ($N_{CP}$) for each platform using different combination methods and user-defined weights. }}
\label{tab:ncp-score-table-norm}
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{\textbf{Platform}} &
$S_{max}$ & $S_{map}$ & $S_{zsc}$ & $S_{sum}$ & $P$ & $N_{AL}$ \\ \midrule
UAS A & 0.238 (7) & 0.185 (7) & -0.982 (7) & 0.062 (7) & 3.173 (7) & 3\\ 
UAS B & 0.431 (4) & 0.427 (3) &	-0.084 (4) & 0.116 (3) & 4.658 (4) & 1\\ 
UAS C & 0.387 (6) & 0.335 (6) & -0.138 (6) & 0.106 (6) & 4.512 (5) & 0\\ 
UAS D & 0.479 (2) & 0.472 (2) & 0.014 (3) & 0.125 (2) & 5.355 (2) & 3\\ 
UAS E & 0.781 (1) & 0.856 (1) & 1.278 (1) & 0.208 (1) & 8.508 (1) & 3	\\ 
UAS F & 0.443 (3) & 0.427 (4) & -0.097 (5) & 0.114 (4) & 5.006 (3) & 0	\\ 
UAS G & 0.420 (5) & 0.381 (5) &	0.159 (2) & 0.109 (5) & 4.385 (6) & 0\\
\bottomrule
\end{tabular}
\end{table}
%\end{minipage}

\end{comment}



\begin{comment}

\vspace{-1em}
\hspace{\fill}
\vspace{-1em}
\begin{minipage}{.45\linewidth}
\centering
\scriptsize
\caption{\small{UAS platform rankings based on $N_{CP}$ scores obtained by different combining methods using user-defined weights.}}
\label{tab:ncp-rankings-table}
\begin{tabular}{lccccc}
\toprule
\multicolumn{1}{c}{\textbf{Platform}} &
$S_{max}$ & $S_{map}$ & $S_{zsc}$ & $S_{sum}$ & $P$
\\ \midrule
UAS A & 6 &  6 & 6 & 6 & 6 \\
UAS B & 5 & 4 & 3 & 3 & 4 \\ 
UAS D & 2 & 2 & 2 & 2 & 2 \\ 
UAS E & 1 & 1 & 1 & 1 & 1	\\ 
UAS F & 3 & 3 & 4 & 4 & 3	\\ 
UAS G & 4 & 5 & 5 & 5 & 5\\ 
\bottomrule

\end{tabular}
\end{minipage}
%\end{table}
\end{comment}
%\vspace{-1em}



\begin{comment}

\begin{figure}[h]
\centering
\includegraphics[width=0.10\textwidth]{Figures/radial_plots/autonomy_plot_legend.png}
\includegraphics[width=0.17\textwidth]{Figures/radial_plots/autonomy_rad_plots1.png}
\includegraphics[width=0.17\textwidth]{Figures/radial_plots/autonomy_rad_plots2.png}
\includegraphics[width=0.17\textwidth]{Figures/radial_plots/autonomy_rad_plots3.png}
\includegraphics[width=0.17\textwidth]{Figures/radial_plots/autonomy_rad_plots4.png}
\includegraphics[width=0.17\textwidth]{Figures/radial_plots/autonomy_rad_plots5.png}
\caption{\small{Autonomy evaluations of the systems using polar plots. In each plot, $N_{AL}$ is shown as the radius and $N_{CP}$ is the angle from the x-axis. Evaluations here are from uniform weights.}}
\label{fig:radial-chart}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.10\textwidth]{Figures/radial_plots/autonomy_plot_legend.png}
\includegraphics[width=0.17\textwidth]{Figures/radial_plots/autonomy_rad_plots_new_weights1.png}
\includegraphics[width=0.17\textwidth]{Figures/radial_plots/autonomy_rad_plots_new_weights2.png}
\includegraphics[width=0.17\textwidth]{Figures/radial_plots/autonomy_rad_plots_new_weights3.png}
\includegraphics[width=0.17\textwidth]{Figures/radial_plots/autonomy_rad_plots_new_weights4.png}
\includegraphics[width=0.17\textwidth]{Figures/radial_plots/autonomy_rad_plots_new_weights5.png}
\caption{\small{Autonomy evaluations of the systems using polar plots. In each plot, $N_{AL}$ is shown as the radius and $N_{CP}$ is the angle from the x-axis. Evaluations here are from user-defined weights.}}
\label{fig:radial-user-chart}
\end{figure}
\end{comment}

\begin{comment}

\begin{figure}[h]
\centering
\includegraphics[width=0.6\textwidth]{Figures/ncp_rankings_AO.png}
\end{figure}

\end{comment}

